Diffusion Models for Graphs Benefit From Discrete State Spaces

Denoising diffusion probabilistic models and score-matching models have proven to be very powerful for generative tasks. While these approaches have also been applied to the generation of discrete graphs, they have, so far, relied on continuous Gaussian perturbations. Instead, in this work, we suggest using discrete noise for the forward Markov process. This ensures that in every intermediate step the graph remains discrete. Compared to the previous approach, our experimental results on four datasets and multiple architectures show that using a discrete noising process results in higher quality generated samples indicated with an average MMDs reduced by a factor of 1.5. Furthermore, the number of denoising steps is reduced from 1000 to 32 steps, leading to a 30 times faster sampling procedure.

==> ddsg4.tex <==
\subsection{Sampling}\label{sec:sampling}
For each loss, we used a specific sampling algorithm. For both approaches, we start by sampling each edge independently from a Bernoulli distribution with probability $p=1/2$ (Erdős–Rényi random graph). Then, for the $L_{\text{vb}}$ loss we follow \citet{ho2020denoising} and iteratively reverse the chain by sampling Bernoulli-sampling from $p_{\theta}(\bm{A}_{t-1} \mid \bm{A}_{t})$ until we obtain our sample of $p_{\theta}(\bm{A}_{0} \mid \bm{A}_{1})$.
For the loss function $L_{\text{simple}}$, we sample $\bm{A}_{0}$ directly from $p_{\theta}(\bm{A}_{0}|\bm{A}_{t})$ for each step t and obtain $\bm{A}_{t-1}$ by sampling again from $q(\bm{A}_{t-1} \mid \bm{A}_{0})$. The two approaches are described algorithmically in Appendix~\ref{appx:sampling}.
% in Algorithms~\ref{algorithm_vb} and~\ref{algorithm_simple}.

% Noise schedule
The values of $\bar{\beta}_t$ are selected following a simple linear schedule for our reverse process \citep{sohl2015deep}
% as originally proposed by \citet{sohl2015deep}
. We found it works similarly well as other options such as cosine schedule~\citep{nichol2021improved}. Note that in this case $\beta_t$ can be obtained from $\bar{\beta}_t$ in a straightforward manner (see Appendix~\ref{appx:beta_bar}).



==> experiment.tex <==
% 
% Models (+ noise conditioning)
We compare our graph discrete diffusion approach to the original score-based approach proposed by \citet{pmlr-v108-niu20a}.
Models using this original formulation are denoted by \textit{score}. 
We follow the training and evaluation setup used by previous contributions \cite{you2018graphrnn,liu2019graph,pmlr-v108-niu20a,jo2022score}. More details can be found in Appendix~\ref{appx:training_setup}.
For evaluation, we compute MMD metrics from~\cite{you2018graphrnn} between the generated graphs and the test set, namely, the degree distribution, the clustering coefficient, and the 4-node orbit counts. To demonstrate the efficiency of the discrete parameterization, the discrete models only use $32$ denoising steps, while the score-based models use $1000$ denoising steps, as originally proposed.
We compare two architectures: 1. EDP-GNN as introduced by \citet{pmlr-v108-niu20a}, and 2. a simpler and more expressive provably powerful graph network (PPGN)~\citep{maron2019provably}. See Appendix~\ref{appx:models} for a more detailed description of the architectures. 
The code is publicly available\footnote{\url{https://github.com/kilian888/discrete_DPPM_Graphs/}}.

\begin{wraptable}{r}{.55\linewidth}
\vspace{-0.35cm}
\scalebox{0.57}{
    \centering
    \begin{tabular}{lccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Community}} & \multicolumn{5}{c}{\textbf{Ego}} \\
    \cmidrule(rl){2-5} \cmidrule(rl){6-9}
    \textbf{Model} & {Deg.} & {Clus.} & {Orb.} & {Avg.} & {Deg.} & {Clus.} & {Orb.} & {Avg.} & {Total} \\
    \midrule
    GraphRNN$^{\dagger}$ & 0.030 & 0.030 & 0.010 & \textbf{0.017} & 0.040 & 0.050 & 0.060 & 0.050 & 0.033 \\
    GNF$^{\dagger}$ & 0.120 & 0.150 & 0.020 & 0.097 & 0.010 & 0.030 & 0.001 & 0.014 & 0.055 \\
    EDP-Score$^{\dagger}$ & 0.006 & 0.127 & 0.018 & 0.050 & 0.010 & 0.025 & 0.003 & \textbf{0.013} & 0.031 \\
    SDE-Score$^{\dagger}$ & 0.045 & 0.086 & 0.007 & 0.046 & 0.021 & 0.024 & 0.007 & 0.017 & 0.032 \\
    \midrule
    EDP-Score\footnotemark
    & 0.016 & 0.810 & 0.110 & 0.320 & 0.04 & 0.064 & 0.005 & 0.037 & 0.178 \\
    PPGN-Score & 0.081 & 0.237 & 0.284 & 0.200 & 0.019 & 0.049 & 0.005 & 0.025 & 0.113 \\
    \midrule
    PPGN $L_{\text{vb}}$ & 0.023 & 0.061 &  0.015 & 0.033 & 0.025 & 0.039 & 0.019 & 0.027 & 0.03 \\
    PPGN $L_{\text{simple}}$ & 0.019 & 0.044 & 0.005 & 0.023 &  0.018 & 0.026 & 0.003 & 0.016 & \textbf{0.019} \\
    \midrule
    EDP $L_{\text{simple}}$ & 0.024 & 0.04 & 0.012 & 0.026 &  0.019 & 0.031 & 0.017 & 0.022 & 0.024 \\
    \bottomrule
    \end{tabular}}
\caption{MMD results for the Community and the Ego datasets. All values are averaged over 5 runs with 1024 generated samples without any sub-selection. 
The "Total" column denotes the average MMD over all of the 6 measurements. The best results of the "Avg." and "Total" columns are shown in bold. 
$\dagger$ marks the results taken from the original papers.
% Results taken from the original papers are indicated with $\dagger$.
\label{tab:results-comunity-ego}}
\scalebox{0.55}{
    \centering
    \begin{tabular}{lccccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{SBM-27}} & \multicolumn{8}{c}{\textbf{Planar-60}} \\
    \cmidrule(rl){2-5} \cmidrule(rl){6-9}
    \textbf{Model} & {Deg.} & {Clus.} & {Orb.} & {Avg.} & {Deg.} & {Clus.} & {Orb.} & {Avg.} & {Total} \\
    \midrule
    EDP-Score    & 0.014 & 0.800 & 0.190 & 0.334 & 1.360 & 1.904 & 0.534 & 1.266 & 0.8 \\
    \midrule
    PPGN $L_{\text{simple}}$ & 0.007 & 0.035 & 0.072 & \textbf{0.038} & 0.029 & 0.039 & 0.036 &  \textbf{0.035} &  \textbf{0.036}\\
    \midrule
    EDP $L_{\text{simple}}$ & 0.046 & 0.184 &0.064 & 0.098 & 0.017 & 1.928 & 0.785 & 0.910 & 0.504\\
    \bottomrule
    \end{tabular}}
\caption{ MMD results for the SBM-27 and the Planar-60 datasets. 
\label{tab:results-planar-sbm}}
% \vspace{-0.25cm}
\end{wraptable} 
\footnotetext{The discrepancy with the EDP-Score$^{\dagger}$ results comes from the fact that using the code provided by the authors, we were unable to reproduce their results. Strangely, their code leads to good results when used with our discrete formulation and $L_{\text{simple}}$ loss improving over the result reported in their contribution.} 
Table~\ref{tab:results-comunity-ego} shows the results for two datasets, Community-small $(12\leq n\leq 20)$ and Ego-small $(4\leq n\leq 18)$, used by \citet{pmlr-v108-niu20a}. 
%These datasets are comprised of relatively small graphs. 
To better compare our approach to traditional score-based graph generation, in Table~\ref{tab:results-planar-sbm}, we additionally perform experiments on slightly more challenging datasets with larger graphs. Namely, a stochastic-block-model (SBM) dataset with three communities, which in total consists of ($24\leq n\leq 27$) nodes and a planar dataset with ($n=60$) nodes. Detailed information on the datasets can be found in the Appendix~\ref{appx:datasets}. Additional details concerning the evaluation setup
% for the different methods
are provided in Appendix~\ref{appx:results-details}.

\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-0.35cm}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/ablation.pdf}
  \end{center}
  \caption{Average MMD compared to the number of denoising steps used on the Ego dataset for PPGN $L_{\text{simple}}$, which uses discrete noise and PPGN-Score, which uses Gaussian noise.}
  \label{fig:ablation}
 \vspace{-0.5cm}
\end{wrapfigure}

\paragraph{Results.}
In Table~\ref{tab:results-comunity-ego}, we observe that the proposed discrete diffusion process using the $L_\text{vb}$ loss and PPGN model leads to slightly improved average MMDs over the competitors. The $L_\text{simple}$ loss further improve the result over $L_\text{vb}$. The fact that the EDP-$L_\text{simple}$ model has significantly lower MMD values than the EDP-score model is a strong indication that the proposed loss and the discrete formulation are the cause of the improvement rather than the PPGN architecture. This improvement comes with the additional benefit that sampling is greatly accelerated (30 times) as the number of timesteps is reduced from 1000 to 32. Table~\ref{tab:results-planar-sbm} shows that the proposed discrete formulation is even more beneficial when the size and complexity of the graph increase. The PPGN-Score even becomes infeasible to run in this setting, due to the prohibitively expensive sampling procedure.
A qualitative evaluation of the generated graphs is performed in Appendix~\ref{appx:samples}. Visually, the $L_\text{simple}$ loss leads to the best samples.


To further showcase the performance improvement of using discrete diffusion, we performed a study on how the number of sampling steps influences the generated sample quality for PPGN $L_{\text{simple}}$, which uses discrete noise, and PPGN-Score, which uses Gaussian noise. In Figure~\ref{fig:ablation} we can see that our model using discrete noise already achieves the best generation quality with just 48 denoising steps, while the model with Gaussian noise achieves worse results even after 1024 steps.



==> related_work.tex <==
% Traditionally, graph generation has been studied through the lens of random graph models~\cite{erdos1960evolution,holland1983stochastic,eldridge2016graphons}. While this approach is insufficient to model many real-world graph distributions, it is useful to create synthetic datasets and provides a useful abstraction. In fact, we will use Erdős–Rényi graphs~\cite{erdos1960evolution} to model the prior distribution of our diffusion process.

% Due to their larger number of parameters and expressive power, deep generative models have achieved better results in modeling complex graph distributions. The most successful graph generative models can be divided into two different techniques: a) auto-regressive graph generative models, which generate the graph sequentially node-by-node \citep{you2018graphrnn, liao2019efficient}, and b) one-shot generative models which generate the whole graph in a single forward pass \citep{simonovsky2018graphvae, de2018molgan, liu2019graph, krawczuk2020gg,  pmlr-v108-niu20a, jo2022score, martinkus2022spectre}. While auto-regressive models can generate graphs with hundreds or even thousands of nodes, they can suffer from mode collapse \cite{krawczuk2020gg, martinkus2022spectre}. One-shot graph generative models are more resilient to mode collapse but are more challenging to train while still not scaling easily beyond tens of nodes. Recently, one-shot generation has been scaled up to graphs of hundreds of nodes thanks to spectral conditioning \citep{martinkus2022spectre}, suggesting that good conditioning can largely benefit graph generation. Still, the suggested training procedure is cumbersome as it involves 3 different intertwined Generative Adversarial Networks (GANs). Finally, Variational Auto Encoders (VAE) have also been studied to generate graphs but remain difficult to train, as the loss function needs to be permutation invariant \citep{vignac2022top} which can necessitate an expensive graph matching step \citep{simonovsky2018graphvae}. 

% In contrast, the score-based models \cite{pmlr-v108-niu20a, jo2022score} have the potential to provide both, a simple, stable training objective similar to the auto-regressive models and good graph distribution coverage provided by the one-shot models. \citet{pmlr-v108-niu20a} provided the first score-based model for graph generation by directly using the score-based model formulation by \citet{song2019generative} and additionally accounting for the permutation equivariance of graphs. \citet{jo2022score} extended this to featured graph generation, by formulating the problem as a system of two stochastic differential equations, one for feature generation and one for adjacency generation. The graph and the features are then generated in parallel. This approach provided promising results for molecule generation. Results on slightly larger graphs were also improved but remained imperfect.
% % although performance on larger graphs was still lacking.
% Importantly, both contributions rely on a continuous Gaussian noise process and use a thousand denoising steps to achieve good results, which makes for a slow graph generation.

% As shown by \citet{song2021scorebased}, score matching is tightly related to denoising diffusion probabilistic models \citep{ho2020denoising} which provide a more flexible formulation, more easily amendable for the graph generation. In particular, for the noisy samples to remain discrete graphs, the perturbations need to be discrete. Such discrete diffusion has been successfully used for quantized image generation \citep{bond2021unleashing, esser2021imagebart} and text generation \citep{hoogeboom2022autoregressive}.
% Diffusion using the multinomial distribution was proposed in \citet{hoogeboom2021argmax}.
% Then, \citet{austin2021structured} extended the previous work by \citet{hoogeboom2021argmax, song2020denoising} and provided a general recipe for denoising diffusion models in discrete
% state-spaces which mainly requires the specification of a doubly-stochastic Markov transition matrix $\bm{Q}$ which ensures the Markov process conserves probability mass and converges to a stationary distribution. 
% In the next section, we describe a formulation of this perturbation matrix $\bm{Q}$ leading to the Erdős–Rényi random graphs.


Traditionally, graph generation has been studied through the lens of random graph models~\cite{erdos1960evolution,holland1983stochastic,eldridge2016graphons}. However, due to the complexity of the graph generation problem, deep generative models have achieved better results. The most successful graph generative models can be divided into two different techniques: a) auto-regressive graph generative models, which generate the graph sequentially node-by-node \citep{you2018graphrnn, liao2019efficient}; b) one-shot generative models, which generate the whole graph in a single forward pass \citep{simonovsky2018graphvae, de2018molgan, liu2019graph, krawczuk2020gg,  pmlr-v108-niu20a, jo2022score, martinkus2022spectre}. While auto-regressive models can generate graphs with hundreds or even thousands of nodes, they can suffer from mode collapse \cite{krawczuk2020gg, martinkus2022spectre}. 
Finally, graph Variational Auto Encoders (VAEs) remain difficult to train, as the loss function needs to be permutation invariant \citep{vignac2022top} which can necessitate an expensive graph matching step \citep{simonovsky2018graphvae}. 

In contrast, the score-based models \cite{pmlr-v108-niu20a, jo2022score} have the potential to provide both a simple, stable training objective similar to the auto-regressive models and good graph distribution coverage provided by the one-shot models. \citet{pmlr-v108-niu20a} provided the first score-based model for graph generation (directly using the score-based model formulation by \citet{song2019generative}). \citet{jo2022score} extended this to featured graph generation, which lead to promising results for molecule generation. 
Importantly, both contributions rely on a continuous Gaussian noise process and use a thousand denoising steps to achieve good results, which makes for a slow graph generation.

As shown by \citet{song2021scorebased}, score matching is tightly related to denoising diffusion probabilistic models \citep{ho2020denoising} that provide a more flexible formulation and are more easily amendable for graph generation. In particular, for noisy samples to remain discrete graphs, the perturbations need to be discrete. Discrete diffusion, using multinomial distribution, was proposed in \citet{hoogeboom2021argmax} and then extended in \citet{austin2021structured}. It has been successfully used for quantized image generation \citep{bond2021unleashing, esser2021imagebart} and text generation \citep{hoogeboom2022autoregressive}.
A new and concurrent work by \citet{vignac2022digress} also investigates discrete DDPM for graph generation and confirms the benefits we outline in this paper.
% After our submission, we became aware of a simultaneous contribution \cite{vignac2022digress} that applies discrete DDPM for graph generation.
% In the next section, we use the formulation of \citet{austin2021structured} to build a forward noising process leading to the Erdős–Rényi random graphs. 

